Variational Selective Autoencoder: Learning from Partially-Observed Heterogeneous Data

Learning from heterogeneous data poses challenges such as combining data from various sources and of different types. Meanwhile, heterogeneous data are often associated with missingness in real-world applications due to heterogeneity and noise of input sources. In this work, we propose the variational selective autoencoder (VSAE), a general framework to learn representations from partially-observed heterogeneous data. VSAE learns the latent dependencies in heterogeneous data by modeling the joint distribution of observed data, unobserved data, and the imputation mask which represents how the data are missing. It results in a unified model for various downstream tasks including data generation and imputation. Evaluation on both low-dimensional and high-dimensional heterogeneous datasets for these two tasks shows improvement over state-of-the-art models.

==> chapters/EMwVI.tex <==

\appendix
\section{Appendix}
In general, we want to maximize complete log-likelihood $\log p(\x_\oo, \x_\uu, \mm|\boldsymbol{\theta}, \boldsymbol{\epsilon})$, where $\boldsymbol{\theta}$ and $\boldsymbol{\epsilon}$ are parameters of data / mask generative models. 
 We have ELBO (Eq.~(\ref{eq:elbo_final})) that lower bounds the complete data log-likelihood and let's treat unobserved $\x_\uu$ as latent variables used in EM.
 
Next we introduce a distribution $q(\x_\uu)$ defined over the unobserved attributes. For any choice of $q(\x_\uu)$, the following decomposition holds,

\begin{align}
    \log p&(\x_\oo, \x_\uu, \mm|\boldsymbol{\theta}, \boldsymbol{\epsilon})
    = \\
    &\mathcal{L}(q| \boldsymbol{\theta}, \boldsymbol{\epsilon}) + D_\text{KL}(q || p(\x_\uu|\x_\oo, \mm, \boldsymbol{\theta}, \boldsymbol{\epsilon}))
\end{align}

where 
\begin{align*}
    \mathcal{L}(q| \boldsymbol{\theta}, \boldsymbol{\epsilon})
    &=\int q(\x_\uu) \log p(\x_\uu,\x_\oo,\mm|\boldsymbol{\theta}, \boldsymbol{\epsilon}) d \x_\uu \\
    &+ \int q(\x_\uu) \log q(\x_\uu) d \x_\uu
\end{align*}
 


At $E$ step, fix $\boldsymbol{\theta}, \boldsymbol{\epsilon}$ as $\boldsymbol{\theta}^*, \boldsymbol{\epsilon}^*$, and lower bound

\begin{align*}
    \mathcal{L}(q| \boldsymbol{\theta}^*, \boldsymbol{\epsilon}^*) = 
\log p(\x_\oo, \x_\uu, \mm|\boldsymbol{\theta}^*, \boldsymbol{\epsilon}^*) - D_{KL}
\end{align*}

 Maximum is obtained if the proposal distribution $q^*=p(\x_\uu|\x_\oo, \mm, \boldsymbol{\theta}^*)$, yielding
 
 \begin{align*}
    \mathcal{L}(q^*| \boldsymbol{\theta}^*, \boldsymbol{\epsilon}^*) = 
\log p(\x_\oo, \x_\uu, \mm|\boldsymbol{\theta}^*, \boldsymbol{\epsilon}^*) %\geq \mathcal{L}_{ELBO}(\x_\oo, \x_\uu, \mm|\boldsymbol{\theta}^*, \boldsymbol{\epsilon}^*, \boldsymbol{\phi}, \boldsymbol{\psi})
\end{align*}
 

At $M$ step, fix $q=p(\x_\uu|\x_\oo, \mm, \boldsymbol{\theta}^*)$ and to maximize lower bound w.r.t parameters:

\begin{align*}
    \mathcal{L}(q^*| \boldsymbol{\theta}, \boldsymbol{\epsilon}) &= 
\int q^*(\x_\uu) \log p(\x_\uu,\x_\oo,\mm|\boldsymbol{\theta}, \boldsymbol{\epsilon}) d \x_\uu 
   \\& + \int q^*(\x_\uu) \log q^*(\x_\uu) d \x_\uu 
\end{align*}

The second term of RHS does not depend on $\boldsymbol{\theta}, \boldsymbol{\epsilon}$ therefore equivalent to maximize the first term of RHS. As we derived in varitional inference that $\log p(\x_\uu,\x_\oo,\mm|\boldsymbol{\theta}, \boldsymbol{\epsilon})\geq \mathcal{L}_{\boldsymbol{\phi}, \boldsymbol{\psi}, \boldsymbol{\boldsymbol{\theta}}, \boldsymbol{\boldsymbol{\epsilon}}}(\x_\mathbf{o},\x_\mathbf{u},\mathbf{m}) $, where $\boldsymbol{\phi}, \boldsymbol{\psi}$ are parameters of proposal distribution of variational inference, we have:


\begin{align*}
&\int q^*(\x_\uu) \log p(\x_\uu,\x_\oo,\mm|\boldsymbol{\theta}, \boldsymbol{\epsilon}) d \x_\uu 
   \\&\geq  \int q^*(\x_\uu) \mathcal{L}_{\boldsymbol{\phi}, \boldsymbol{\psi}, \boldsymbol{\boldsymbol{\theta}}, \boldsymbol{\boldsymbol{\epsilon}}}(\x_\mathbf{o},\x_\mathbf{u},\mathbf{m}) d \x_\uu 
\end{align*}

If we generate $\x_\uu$ from $q^*(\x_\uu)=p(\x_\uu|\x_\oo, \mm, \boldsymbol{\theta}^*)\approx
    \int p_{\boldsymbol{\theta}^*}(\x_{\mathbf{u}}|\mathbf{m},\mathbf{z})
    q_{\boldsymbol{\phi}^*,\boldsymbol{\psi}^*}(\mathbf{z}|\x_{\mathbf{o}},\mathbf{m}) d\mathbf{z}$, this holds for standard EM methods. However, 
    if we generate $\x_\uu$ from prior that $
    \int p_{\boldsymbol{\theta}^*}(\x_{\mathbf{u}}|\mathbf{m},\mathbf{z})
    p(\zz) d\mathbf{z}$, $\x_\uu$ is not conditional on $\x_\oo$ but only $\mm$, it might violate the derivation from EM. 

